Decoupling Content and Expression: Two-Dimensional Detection of AI-Generated Text

The wide usage of LLMs raises critical requirements on detecting AI participation in texts. Existing studies investigate these detections in scattered contexts, leaving a systematic and unified approach unexplored. In this paper, we present HART, a hierarchical framework of AI risk levels, each corresponding to a detection task. To address these tasks, we propose a novel 2D Detection Method, decoupling a text into content and language expression. Our findings show that content is resistant to surface-level changes, which can serve as a key feature for detection. Experiments demonstrate that 2D method significantly outperforms existing detectors, achieving an AUROC improvement from 0.705 to 0.849 for level-2 detection and from 0.807 to 0.886 for RAID. We release our data and code at https://github.com/baoguangsheng/truth-mirror.

==> figures/2d_detection.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0pt 5pt 0pt 10pt},clip,width=1.0\linewidth]{sources/2d_detection.pdf}   
    \caption{Content-language coordinate system mapping to AI risk levels.}
    \label{fig:2d_detection}
\end{figure}


==> figures/2d_detection_task.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[trim={0pt 0pt 0pt 0pt},clip,width=1.0\linewidth]{sources/2d_detection_task.pdf}   
    \caption{2D detection tasks and benchmark dataset (M-LAIR).}
    \label{fig:2d_detection_task}
\end{figure*}

==> figures/2d_distribution_details.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={25pt 0pt 40pt 0pt},clip,width=1.0\linewidth]{sources/distrib_content_language.details.pdf}   
    \caption{2D distribution details.}
    \label{fig:2d_distribution2}
\end{figure}



==> figures/benchmark_coverage.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={50pt 0pt 70pt 0pt},clip,width=1.0\linewidth]{sources/benchmark_coverage.jpg}   
    \caption{Benchmark coverage.}
    \label{fig:benchmark_coverage}
\end{figure}

==> figures/benchmark_dataset.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0pt 0pt 0pt 0pt},clip,width=1.0\linewidth]{sources/benchmark_dataset.pdf}   
    \caption{Benchmark dataset.}
    \label{fig:benchmark_dataset}
\end{figure}



==> figures/raid_dev_samples_linechart.tex <==
\begin{figure}[t]

\end{figure}



==> tables/results_content_language.tex <==
\begin{table}[t]
    % \vspace{-0.2in}
    \centering\scriptsize
    \begin{tabular}{l|cc|cc}
        \toprule
        \bf Detector & \multicolumn{2}{c|}{\bf AI Content} & \multicolumn{2}{c}{\bf AI Language} \\
        & AUROC & F1 & AUROC & F1 \\
        \midrule
        Log-Perplexity & 0.4940 & 67\% & 0.7690 & 72\% \\
        Fast-Detect & 0.6842 & 66\% & 0.7661 & \bf 73\% \\
        Binoculars & 0.6858 & 68\% & \bf 0.7796 & \bf 73\% \\
        Content (Binoculars) & \bf 0.7850 & \bf 73\% & 0.5637 & 67\% \\
        Language (Binoculars) & 0.6560 & 67\% & 0.7188 & 68\% \\
        2D-CL (Binoculars) & 0.8249 & 77\% & 0.7366 & 68\% \\
        2D-CG (Binoculars) & \bf 0.8525 & \bf 80\% & \bf 0.8023 & \bf 76\% \\
        \bottomrule
    \end{tabular}
    \caption{Results on AI content and language detection, evaluated on English M-LAIR across Essay, Arxiv, and Writing.}
    \label{tab:results_content_language}
\end{table}

